VIRES: Video Instance Repainting via Sketch and Text Guided Generation

We introduce VIRES, a video instance repainting method with sketch and text guidance, enabling video instance repainting, replacement, generation, and removal. Existing approaches struggle with temporal consistency and accurate alignment with the provided sketch sequence. VIRES leverages the generative priors of text-to-video models to maintain temporal consistency and produce visually pleasing results. We propose the Sequential ControlNet with the standardized self-scaling, which effectively extracts structure layouts and adaptively captures high-contrast sketch details. We further augment the diffusion transformer backbone with the sketch attention to interpret and inject fine-grained sketch semantics. A sketch-aware encoder ensures that repainted results are aligned with the provided sketch sequence. Additionally, we contribute the VireSet, a dataset with detailed annotations tailored for training and evaluating video instance editing methods. Experimental results demonstrate the effectiveness of VIRES, which outperforms state-of-the-art methods in visual quality, temporal consistency, condition alignment, and human ratings. Project page: https://hjzheng.net/projects/VIRES/

==> sec/0_abstract.tex <==
\begin{abstract}
\zpx{placeholder:The Affective Image Filter (AIF), as a novel task that aims at reflecting visually-abstract emotions from texts to visually-concrete images, poses great challenges in both accurate emotional understanding and appropriate emotional visualization. 
 We first introduce the AIF dataset and AIFormer, a multi-modal transformer architecture developed as an initial baseline approach.
 To push AIF models towards \textbf{De}eper \textbf{E}motional \textbf{R}eflection, we propose \textbf{DeER} that leverages generative priors from pre-trained large-scale models. 
 To maintain content consistency and high-frequency details of content images, we design a content preservation module. 
 To accurately understand ambiguous and subjective emotions, we introduce an LLM and CoT prompting to improve emotional understanding and present a voting ensemble mechanism that analyzes evoked emotions accurately.
 To enhance the emotional understanding and to balance artistic style and content consistency while avoiding overly-stylized effects, we propose the artistic mapping strategy.
 Extensive experimental results demonstrate both objective and subjective superiority of DeER over state-of-the-art methods, where DeER exhibits a more accurate emotional understanding of texts and synthesizes corresponding visually appealing images.}
\end{abstract}
%  

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


==> sec/2_relatedwork.tex <==
\section{Related work}
\label{sec:related}



==> sec/3_dataset.tex <==
\section{Dataset}
\label{sec:dataset}


==> sec/4_methodology.tex <==
\section{Method}
\label{sec:method}

% overview

% pretrain VAE

% 


==> sec/5_experiment.tex <==

\section{Experiments}

\subsection{Comparison}
\subsection{Ablation}
\subsection{User study}

==> sec/6_discussion.tex <==
\section{Discussion}




==> sec/7_conclusion.tex <==
\section{Conclusion}


\clearpage


